Adaptive 3D Localization of 2D Freehand Ultrasound Brain Images

Two-dimensional (2D) freehand ultrasound is the mainstay in prenatal care and fetal growth monitoring. The task of matching corresponding cross-sectional planes in the 3D anatomy for a given 2D ultrasound brain scan is essential in freehand scanning, but challenging. We propose AdLocUI, a framework that Adaptively Localizes 2D Ultrasound Images in the 3D anatomical atlas without using any external tracking sensor.. We first train a convolutional neural network with 2D slices sampled from co-aligned 3D ultrasound volumes to predict their locations in the 3D anatomical atlas. Next, we fine-tune it with 2D freehand ultrasound images using a novel unsupervised cycle consistency, which utilizes the fact that the overall displacement of a sequence of images in the 3D anatomical atlas is equal to the displacement from the first image to the last in that sequence. We demonstrate that AdLocUI can adapt to three different ultrasound datasets, acquired with different machines and protocols, and achieves significantly better localization accuracy than the baselines. AdLocUI can be used for sensorless 2D freehand ultrasound guidance by the bedside. The source code is available at https://github.com/pakheiyeung/AdLocUI.

==> sec/02-preliminary.tex <==

% ====================
% Preliminary
% ====================
% \vspace{-5pt}
\section{Construction of 3D Representations}
\label{sec:preliminary}
In Section~\ref{sec:representation},
we briefly review the two ways of representing a 3D volume,
followed by the conventional 3D reconstruction approaches,
and our proposed approach with implicit representation in Section~\ref{sec:conventional}.


% ====================
% Explicit and Implicit 3D Representations
% ====================
\subsection{Explicit and Implicit 3D Representations}
\label{sec:representation}
The very nature of a 3D volume is a one-to-one mapping from a set of 3D space positions (\ie 3D coordinates) to the corresponding intensity values in real world.
In general, there are two different ways for representing a 3D volume, 
either \emph{explicitly} or \emph{implicitly},
as described and compared in Table~\ref{table:preliminary} and the following sections:
% ====================
% Table - Preliminary
% ====================
\input{sec/table_preliminary}
\\[-8pt]
\par{\noindent \bf Explicit Representation.}
Conventionally, 
a 3D volume, $\mathbf{V} \in \mathcal{R}^{H \times W \times D \times C}$,
is represented \emph{discretely} and \emph{explicitly} as a tensor with height ($H$), width ($W$), depth ($D$), and intensity channels~($C$).
Most medical applications involving 3D volumes rely on using such representation. 
\\[-6pt]
    
\par{\noindent \bf Implicit Representation.}
As an alternative,
a 3D volume can also be represented as a zero level set of a {\em continuous} 
function parameterized by $\mathrm{\Theta}$.
Such {\em implicit} representation compresses the volumetric information
and encodes it as parameters of a model, 
for example a deep neural network,
that maps the 3D coordinates, $\mathbf{x} = (x, y, z)$, to intensities,
{\ie}~$F_\mathrm{\Theta} : \mathbf{x} \rightarrow c$.

%With such property, the v
%Its \emph{continuous} nature facilitates our 
%joint optimization as introduced in Section~\ref{sec:conventional} and \ref{sec:optimization},
%contributing to the major boost of performance (Table~\ref{table:result}) achieved by our framework.
% In this work, we adopt such representation and parameterize the function, $F_\mathrm{\Theta}$, by a deep neural network.


% ====================
% Conventional 3D Reconstruction Approaches
% ====================
\subsection{Conventional 3D Reconstruction Approaches}
\label{sec:conventional}

In the literature,
as summarized in \cite{mohamed2019survey},
early attempts on 2D-to-3D ultrasound reconstruction have been extensively built on the explicit representations, 
and can be summarised by the following steps: 
% as summarized below:

\begin{itemize}
\item[$\bullet$] First, 
the 3D location of each 2D ultrasound image is estimated,
where external sensor tracking is required at either the \emph{training}~\cite{prager2003sensorless, prevost2017deep} or \emph{inference}~\cite{daoud2015freehand, chung2017freehand} stage,
subject to errors caused by subjects' internal motion (\eg fetal movement).

\item[$\bullet$] Then,
a 3D volume, 
represented \emph{discretely} as a tensor of intensities,
is reconstructed by `registering' the localized 2D scans back to the 3D space,
with holes being interpolated.
However, such 2D-to-3D back-projections are often  
prone to errors, leading to artifacts,
thus requiring post-hoc corrections.

%which is unavoidable in practice.
% in all sorts of aforementioned 3D location estimation approaches.
% The resulted artifacts can be visualized from \emph{\media} of Fig.~\ref{fig:synthetic}.

\item[$\bullet$] Finally,
approaches~\cite{chen2014reconstruction, moon20163d}
have been proposed to correct the aforementioned reconstruction artifacts,
based on kernel smoothing and denoising.
However the effect may be limited,
as the source of inaccuracy from the localization of the 2D images is unsolved,
which can be visualized in the last two rows of Fig.~\ref{fig:synthetic}.
\end{itemize}



% \weidi{what do these methods do, why not generalisable ? 
% are they doing something like denoising in the image domain ?
% explain it clearly.}


\par{\noindent \bf Contributions.}
In this paper, 
we parametrise a deep neural network for representing a 3D volume implicitly~(Fig.~\ref{fig:pipeline}).
Such a representation is continuous, 
and enables the querying of intensities at arbitrary spatial coordinates. 
With only a set of 2D scans available, 
it can produce jointly optimal 3D structures and 3D location estimations for these scans.

%Our proposed \proposed, using \media for 3D location estimation,
%is \emph{genuine} sensorless in both \emph{training} and \emph{inference} phases.



%Metaphorically,
%the in-garbage (\ie pre-estimated 3D locations) is now gradually refined during training,
%which simultaneously improves the output (\ie reconstruction) quality.

% We represent the 3D volume \emph{implicitly} by a deep neural network,
% which replaces step 2 and 3 
% by simple network training
% from the 2D images (Fig.~\ref{fig:pipeline}).
% The \emph{continuous} implicit representation
% allows joint optimization of the pre-estimated 3D locations of the 2D images while reconstructing the 3D volume (\ie training the network),
% similar to bundle adjustment~\cite{kanatani2011bundle} but in a deep learning manner.
% Metaphorically,
% the in-garbage is now gradually refined during training,
% which simultaneously improves the output (\ie reconstruction) quality.





% % ====================
% % Explicit Representation
% % ====================
% \subsection{Explicit Representation}
% \label{sec:explicit}
% Conventionally, a 3D volume,
% $\mathbf{V} \in \mathcal{R}^{H \times W \times D}$,
% is represented in the form of a discrete voxel grid,
% where $H$, $W$ and $D$ are the height, width and depth of the volume.

% Most of the applications on medical 3D volumes rely on using such representation.
% Nevertheless, the discrete nature endows the explicit representation with several limitations,
% for example 
% the relatively large memory required,
% the resolution constrainted by the grid,
% as well as the difficulties of computing derivatives due to discretization~\cite{sitzmann2020implicit}.
% Therefore, we propose to use implicit representation in this work.


% % ====================
% % Implicit Representation
% % ====================
% \subsection{Implicit Representation}
% \label{sec:implicit}
% In general,
% a 3D volume can be represented \emph{continuously} by a MLP representation network,
% $F_\mathrm{\Theta} : \mathbf{x} \rightarrow c$,
% where $\mathrm{\Theta}$ is the weights of the network
% and $c$ is the volume intensity at any 3D coordinates,
% $\mathbf{x} = (x, y, z)$.

% The \emph{continuous} implicit representation enjoys several advantages over the explicit representation, 
% namely, 
% the ability to model high-resolution details by increasing the capacity of the representation network,
% $F_\mathrm{\Theta}$, which is significantly more memory-efficient,
% as well as the implicit representation's differentiability,
% which makes computation that requires gradients much more feasible~\cite{sitzmann2020implicit}.

% Implicit representation by neural network is proposed recently for 
% novel views synthesis from natural scenes~\cite{sitzmann2019scene, mildenhall2020nerf, wang2021nerfmm}
% and objects and shapes representation~\cite{sitzmann2020implicit}.
% To the best of our knowledge,
% this is the first study to manipulate implicit representation for 3D medical volume reconstruction.



